Greybox XAI: a Neural-Symbolic learning framework to produce interpretable predictions for image classification

Although Deep Neural Networks (DNNs) have great generalization and prediction capabilities, their functioning does not allow a detailed explanation of their behavior. Opaque deep learning models are increasingly used to make important predictions in critical environments, and the danger is that they make and use predictions that cannot be justified or legitimized. Several eXplainable Artificial Intelligence (XAI) methods that separate explanations from machine learning models have emerged, but have shortcomings in faithfulness to the model actual functioning and robustness. As a result, there is a widespread agreement on the importance of endowing Deep Learning models with explanatory capabilities so that they can themselves provide an answer to why a particular prediction was made. First, we address the problem of the lack of universal criteria for XAI by formalizing what an explanation is. We also introduced a set of axioms and definitions to clarify XAI from a mathematical perspective. Finally, we present the Greybox XAI, a framework that composes a DNN and a transparent model thanks to the use of a symbolic Knowledge Base (KB). We extract a KB from the dataset and use it to train a transparent model (i.e., a logistic regression). An encoder-decoder architecture is trained on RGB images to produce an output similar to the KB used by the transparent model. Once the two models are trained independently, they are used compositionally to form an explainable predictive model. We show how this new architecture is accurate and explainable in several datasets.

==> docsetup.tex <==
\usepackage{setspace}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{color}
\usepackage[Lenny]{fncychap}


\usepackage[utf8]{inputenc}

%% Header titles
\usepackage{titlesec}
% lscape.sty Produce landscape pages in a (mainly) portrait document.
\usepackage{lscape}

\usepackage{adjustbox}
\usepackage{multirow}

\usepackage[font=small,labelfont=bf]{caption}
\usepackage{fancyhdr}
\usepackage{times}
%\usepackage[intoc]{nomencl}
%\renewcommand{\nomname}{List of Abbreviations}
%\makenomenclature
\usepackage[
backend=biber,
style=numeric,
citestyle=numeric
]{biblatex}
\addbibresource{mylib.bib}


\usepackage{float}
%\floatstyle{boxed} 
\restylefloat{figure}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{epigraph}

%% REMOVE IF YOU WANT TO CHANGE REF STYLE
\usepackage{apalike}

\usepackage{booktabs}
\usepackage[pdftex,bookmarks=true]{hyperref}
\usepackage[pdftex]{hyperref}

\hypersetup{
    colorlinks,%
    citecolor=blue,%
    filecolor=blue,%
    linkcolor=black,%
    urlcolor=blue
}


\def\bsq#1{ %both single quotes
\lq{#1}\rq}


% ShareLaTeX does not support glossaries now. Sorry...
%\usepackage[number=none]{glossary}
%\makeglossary
%\newglossarytype[abr]{abbr}{abt}{abl}
%\newglossarytype[alg]{acronyms}{acr}{acn}
%\newcommand{\abbrname}{Abbreviations} 
%\newcommand{\shortabbrname}{Abbreviations}
%%\makeabbr
\newcommand{\HRule}{\rule{\linewidth}{0.5mm}}

% \renewcommand*\contentsname{Table of Contents}

% \pagestyle{fancy}
% \fancyhf{}
% \renewcommand{\chaptermark}[1]{\markboth{\chaptername\ \thechapter.\ #1}{}}
% \renewcommand{\sectionmark}[1]{\markright{\thesection\ #1}}
% \renewcommand{\headrulewidth}{0.1ex}
% \renewcommand{\footrulewidth}{0.1ex}
% \fancypagestyle{plain}{\fancyhf{}\fancyfoot[LE,RO]{\thepage}\renewcommand{\headrulewidth}{0ex}}


% %\pagestyle{headings} 

==> internal_discussion.tex <==
\textbf{Case B}: Since we choose $v$ to be $0$ and $v$ has only real values, if $v=0$, we therefore should not backpropagate any error through the loss function, since no BB is detected for the object part. 
% In the negative case, SHAP values and KG values should be of opposite signs for the misattribution to be 0. If they have the same sign, there will be feature misattribution, and its weight will be proportional to the absolute value of the SHAP attribution. 
% We penalize similarly both cases, because we assume that the absence of an element can not contribute positively toward the prediction of one of its supposed macro labels. Therefore, in b), if both the SHAP value and the theoretical (KG) attribution are positive, it means that an attribute should have been detected, and it was not, and therefore, there is a mismatch. 
% Similarly, if the theoretical attribution is negative (i.e., the expert KG indicates that that element does not contribute to that object class), and so is the SHAP value (meaning that the element is typical of this object class), then there is a mismatch. 
% We can not assume how it will affect other macro labels. %N it would require counterfactual explanations of unseen data. Can we drive the data annotation by crafting the kind of examples to be seen and thus, obtain a causal misattribution explanation? 
% Thus, the misattribution function when the feature value is $<=v$ becomes:
% \begin{equation}
%     \beta(S,KG,i,k,j) = (KG_{k,j} \times S_{i,k,j})^+
% \end{equation}
% Example: Consider element $E$ and style $S$. The KG tells us that $E$ is typical of $S$ (theoretical, positive attribution with value +1). Our SHAP analysis produces a negative attribution for $E$ in the case of classifying the instance as class $S$. Thus, it tells us that element $E$ is empirically not typical of $S$. Therefore, there is a misalignment with the KG that should be penalized.
%In practice, since in this particular work, $v = 0$, the second formulation of the misattribution function is irrelevant, as the negative case corresponds to the absence of detection of an element. 

%This means that this second formulation of the misattribution function is not for now used. %\c{Its not very relevant to spend half a page explaining something you don't use ...}% The idea was to make it general keeping value of the object parts detector as a value that can be later variable (ie. also negative), even if we dont do it in this case as it is a crisp value and always with abs value of 1.




% ****
% clarifications

%These were not used in this work. %ToDo Jules 15 architectural elements in the pic, but version using 14. Which one is missing in our experiments? future work, how to integrate them? Natalia In the pic there are only 14 elements right ? The element we don't use is the 'gothic pinacle'.


 %However, for the Pascal part, could we conclude that all detected parts represent better the expert knowledge, as they get better SHAP GED?no because it can be good mAP by chance when the dataset is wrong.
 
 
 summary:    Aggregation of Faster vs Retina is different by design: the aggregation function used in faster RCNN is a sum after the NMS: The output of RCNN is a list of the form [(x1,x2,y1,y2,class,confidence), ...] What they do is the sum together the confidence of elements having the same class and put it in a vector. All values used are the default ones of torchvision for my part. In Faster it is confidence comes from the class. 
  % Retina uses the sum, but the batch is of size 1, when changing it, the size of the image is too big, I don't know why I got out of memory which seems to come from the StyleClassificationModel module and behaves badly for unknown reasons. 
  
  
 
 [15:45, 1/11/2021] Natalia: "Vector v aggregates the confidence of each predicted object-part. " predicted by the different region proposals of which model? can I complete this sentence this way?
[16:56, 1/11/2021] Jules Sanchez: Yes it seems weird let me check
[17:02, 1/11/2021] Jules Sanchez: So it is the formula extracted from the DeLDECAS draft, and applies to FasterRCNN
[17:03, 1/11/2021] Jules Sanchez: Here is the extract from the paper
[17:04, 1/11/2021] Jules Sanchez: But I think the formula for RetinaNet would be the same, it just that p_j is different from 0 for more that one value of i
[17:20, 1/11/2021] Natalia: isnt this related to the sum vs max aggregating function then? both do Sum the elements then?
[17:21, 1/11/2021] Natalia: Gianni was investigating this
[17:21, 1/11/2021] Jules Sanchez: There is an implicit max for fasterRCNN. That comes from the ouput of FasterRCNN
[17:21, 1/11/2021] Jules Sanchez: It gives only the scores of the most likely class
[17:21, 1/11/2021] Jules Sanchez: And discards everything else
[17:27, 1/11/2021] Gianni Franchi: hello sorry I am working as an emergency reviewer for CVPR
[17:35, 1/11/2021] Gianni Franchi: I have some difficulties with the faster RCNN codes that mixes pytorch and tensorflow.         
matrix_metadata = metadata_to_matrix(TMP_TRAIN, "json")
        names = matrix_metadata[:,-1]
        train_data = np.zeros((len(names),num_archi_features))
        train_label = np.zeros(len(names))
        if data == "MonumenAI":
            for i in range(len(names)):
                im_name = names[i][2:-4]
                idx = train_loader.images_loc['path'].str.contains(im_name)
                train_data[idx] = matrix_metadata[i,:num_archi_features]
                train_label[idx] = matrix_metadata[i,num_archi_features]

        #Initialize model
        classificator = keras.Sequential()
        classificator.add(keras.layers.Dense(units=n_neurons_classi…
[17:36, 1/11/2021] Gianni Franchi: while for retinanet it is of 1. I try but it is impossible to change it...
[17:36, 1/11/2021] Jules Sanchez: Sadly. Here is the reason RetinaNet came in the first poace
[17:37, 1/11/2021] Gianni Franchi: regarding the aggregation function for Retinanet the definition of the proba is different than the one of faster RCNN hence it is impossible to define the exact same aggregation function.
[17:37, 1/11/2021] Jules Sanchez: I don't do the matrix medata computation
[17:37, 1/11/2021] Jules Sanchez: It's feom grenada team
[17:37, 1/11/2021] Gianni Franchi: oh no..... ok then then they aggregate to increase the batchsize
[17:38, 1/11/2021] Jules Sanchez: I know what should be computed. But not sure the exact process
[17:38, 1/11/2021] Jules Sanchez: Lemme check retinanet for classification
[17:38, 1/11/2021] Gianni Franchi: lemme?
[17:38, 1/11/2021] Jules Sanchez: Let me
[17:38, 1/11/2021] Gianni Franchi: who is Lemme?
[17:39, 1/11/2021] Jules Sanchez: Sorry using the usual abbreviations on phone.my bad x)
[17:40, 1/11/2021] Gianni Franchi: no worry!  For Retina it is use the sum I have checked.But the bath is of 1.
[17:40, 1/11/2021] Jules Sanchez: Yes I know. I'm looking at where I hardcoded it was going to be 1
[17:40, 1/11/2021] Jules Sanchez: And how badly I wrote it
[17:41, 1/11/2021] Gianni Franchi: I manage to change it, but it is impossible, the size of the image is too big, I don't know why I got out of memory
[17:41, 1/11/2021] Jules Sanchez: I think it comes from the StyleClassificationModel moduke
[17:42, 1/11/2021] Jules Sanchez: I had already memory issue
[17:42, 1/11/2021] Jules Sanchez: But it is weird
[17:42, 1/11/2021] Jules Sanchez: I'm not sure why it behaves so badly
[17:43, 1/11/2021] Gianni Franchi: To be honnest I don't know.
[17:44, 1/11/2021] Gianni Franchi: Do you understand the aggregation function used in faster RCNN?
[17:44, 1/11/2021] Gianni Franchi: I don't understand it
[17:44, 1/11/2021] Gianni Franchi: sorry
[17:44, 1/11/2021] Jules Sanchez: Yes
[17:44, 1/11/2021] Gianni Franchi: perfect
[17:44, 1/11/2021] Gianni Franchi: it is a sum after the nms?
[17:44, 1/11/2021] Gianni Franchi: which value of Iou did you set?
[17:45, 1/11/2021] Jules Sanchez: Basically. The output of RCNN is a list of the form [(x1,x2,y1,y2,class,confidence), ...]
[17:45, 1/11/2021] Jules Sanchez: What they do is the sum together the confidence of elements having the same class
[17:46, 1/11/2021] Jules Sanchez: And put it in a vector
[17:46, 1/11/2021] Jules Sanchez: All values used are the default one of torchvision for my part
[17:46, 1/11/2021] Gianni Franchi: no for the faster it is confidence comes from the class
[18:07, 1/11/2021] Gianni Franchi: in summury for natalia the aggregation is different I understood how I try to correct for tomorrow




I also agree with Giannini's argument. In addition, mAP evaluate only one part of the model and not the whole model. Therefore, it makes more sense to correlate SHAP-GED with the accuracy of the overall classification model. However, if we compare the old results of RetinaNet with the new ones, it seems that when the accuracy of the overall model increases the SHAP GED decreases.  Although, I would like to dig more into this interesting point, I think that to be practical, we should work on finishing and submitting the manuscript first. Thank you all for the nice work Best regards, Siham El 2021-01-20 00:13, Diaz Rodriguez Natalia escribió: > hi Siham and Alberto, >  here last experiments of Gianni, in the most fair way he could (same > aggregating function, he could not have time to learn using a new > cluster and so runned it with batch size 1), see email below. >  Do you agree with this explanation? > > Natalia DIAZ RODRIGUEZ > > Enseignant chercheur > > Téléphone : 01 81 87 20 51 > > ------------------------- > > ENSTA Paris | Institut Polytechnique de Paris > > 828 boulevard des Maréchaux > > 91120 Palaiseau [plan [1]] > > www.ensta-paris.fr ENSTA Paris, une Grande école d&#039;ingénieurs généraliste L’ENSTA Paris délivre une formation pluridisciplinaire correspondant à ses domaines d’excellence : l&#039;industrie automobile, ferroviaire ou navale, l&#039;énergie nucléaire, les énergies renouvelables, la robotique, les mathématiques financières ou l&#039;environnement ; des secteurs en phase avec besoins des grandes entreprises. www.ensta-paris.fr [2] | LinkedIn [3] | Twitter [4] | Facebook [5] | > Instagram [6] > >  [7] > > ------------------------- > > From: Franchi Gianni <gianni.franchi@ensta-paris.fr> > Sent: Tuesday, January 19, 2021 9:39 AM > To: Diaz Rodriguez Natalia <natalia.diaz@ensta-paris.fr>; Jules > Sanchez <jules.n.sanchez@gmail.com> > Subject: new results > >  hello Natalia, > > Here is the results I get: > Results on MONU AI > > ~ & mAP & Accuracy &SHAP GED >  Faster R-CNN & $42.5$ & $86.8$ & $0.93$\\ >     \hline >  RetinaNet (OLD results) &  $43.6$ & $87.3$ & $0.59$\\ >  RetinaNet (NEW results) &  $49.5$ & $90.4$ & $0.86$\\ > > Result on Pascal part > ~ & mAP & Accuracy &SHAP GED >  Faster R-CNN &  $36.5$ & $82.4$ & $0.45$\\ >     \hline >  RetinaNet (OLD results) &  $26.5$ & $79.7$ & $0.32$\\  RetinaNet (NEW > results) &  $39.3$ & $80.3$ & $0.59$\\ > >  I think now the results are better. since the accuracy is linked with > the shap GED, but not the mAP. >  This is in coherence with the fact that I dont think the more > accurate the detector is (better mAP) => better GED, >  because the mAP evaluates the spatial location AND the presence or > not of a descriptor, while the GED evelautes just the presence. > 91120 Palaiseau [plan [1]] > > www.ensta-paris.fr [2] | LinkedIn [3] | Twitter [4] | Facebook [5] | > Instagram [6] > >  [7] > > Links: > ------ > [1]  Alberto Castillo Lamas <alcasla90@gmail.com> Wed 1/20/2021 8:18 AM Yes, I agree with Gianni's opinion. mAP evaluation is wider than GED. Moreover, We only take a small batch of detections with confidence above threshold, so no correlation is reasonable.




Thanks for the email Natalia. Maybe I am wrong but I think that from Gianni's results we cannot deduce some correlations between GED, mAP and accuracy. It would be interesting as future work (or now if Gianni has time) to artificially decrease mAp and accuracy and see how GED changes accordingly. This can be performed through ablation studies. What do you think?

A couple of ideas:
* introducing different amount of noise in the training data and check how map, accuracy and GED change accordingly;
* gradually reducing the amount of training data and check how map, accuracy and GED change accordingly;
* ablation studies: turn off some components of EXPLANet (if possible) and check how map, accuracy and GED change accordingly;
Does it sound reasonable?


Ivan

About the fast of adding noise to see the evolution of GED it could be interesting but I don't see the direction to this paper. It would interesting to study GED and how it evolve with mAP and Accuracy and other metrics, but I think that goes behond the scope of the paper.
We could replace Accuracy by Brier Score or Negative log likelihood, or in stead of Map we could use other metrics.

But that is research on metrics
I am sorry but it will be hard for me to conduct these experiments.

best,

Gianni 






About the fast of adding noise to see the evolution of GED it could be interesting but I don't see the direction to this paper. It would interesting to study GED and how it evolve with mAP and Accuracy and other metrics, but I think that goes behond the scope of the paper.
We could replace Accuracy by Brier Score or Negative log likelihood, or in stead of Map we could use other metrics.

But that is research on metrics
I am sorry but it will be hard for me to conduct these experiments.

best,





Gianni FRANCHI

Enseignant chercheur

Téléphone : 01 81 87 20 51

ENSTA Paris | Institut Polytechnique de Paris

828 boulevard des Maréchaux

91120 Palaiseau [plan]

www.ensta-paris.fr | LinkedIn | Twitter | Facebook | Instagram

TA280

De : Diaz Rodriguez Natalia <natalia.diaz@ensta-paris.fr>
Envoyé : mercredi 20 janvier 2021 18:34
À : ivan donadello <donadelloivan@gmail.com>
Cc : Franchi Gianni <gianni.franchi@ensta-paris.fr>
Objet : Re: EXPLANet: new results
 
thanks. +Gianni in cc.

How would you introduce noise to the images and the part labels?
How would you expect the metrics to change accordingly? they are not all correlated always obviously
You have the full architecture of explanet in the paper. What element would you remove for the ablation study?

Gianni wont have time in 10 days deadline for submission I am afraid; Gianni?  if you have, it would be great. Otherwise we ll have to leave it to reviewers' chance.

Natalia DIAZ RODRIGUEZ

Enseignant chercheur

Téléphone : 01 81 87 20 51

ENSTA Paris | Institut Polytechnique de Paris

828 boulevard des Maréchaux

91120 Palaiseau [plan]

www.ensta-paris.fr | LinkedIn | Twitter | Facebook | Instagram

TA280

From: ivan donadello <donadelloivan@gmail.com>
Sent: Wednesday, January 20, 2021 5:16 PM
To: Diaz Rodriguez Natalia <natalia.diaz@ensta-paris.fr>
Subject: Re: EXPLANet: new results
 
A couple of ideas:
introducing different amount of noise in the training data and check how map, accuracy and GED change accordingly;
gradually reducing the amount of training data and check how map, accuracy and GED change accordingly;
ablation studies: turn off some components of EXPLANet (if possible) and check how map, accuracy and GED change accordingly;
Does it sound reasonable?

Il giorno mer 20 gen 2021 alle ore 17:11 Diaz Rodriguez Natalia <natalia.diaz@ensta-paris.fr> ha scritto:
Ita great idea but how would you naturally modify the mAp and accuracy for them to be realistic?

Get Outlook for iOS
From: ivan donadello <donadelloivan@gmail.com>
Sent: Wednesday, January 20, 2021 3:52:41 PM
To: Diaz Rodriguez Natalia <natalia.diaz@ensta-paris.fr>
Subject: Re: Fw: EXPLANet: new results
 
Thanks for the email Natalia. Maybe I am wrong but I think that from Gianni's results we cannot deduce some correlations between GED, mAP and accuracy. It would be interesting as future work (or now if Gianni has time) to artificially decrease mAp and accuracy and see how GED changes accordingly. This can be performed through ablation studies. What do you think?

Ivan

Il giorno mer 20 gen 2021 alle ore 12:59 Diaz Rodriguez Natalia <natalia.diaz@ensta-paris.fr> ha scritto:
what do you think?

Natalia DIAZ RODRIGUEZ

Enseignant chercheur

Téléphone : 01 81 87 20 51

ENSTA Paris | Institut Polytechnique de Paris

828 boulevard des Maréchaux

91120 Palaiseau [plan]

www.ensta-paris.fr | LinkedIn | Twitter | Facebook | Instagram

TA280

From: siham@ugr.es <siham@ugr.es>
Sent: Wednesday, January 20, 2021 9:40 AM
To: Diaz Rodriguez Natalia <natalia.diaz@ensta-paris.fr>
Cc: Alberto Castillo Lamas <alcasla90@gmail.com>; Franchi Gianni <gianni.franchi@ensta-paris.fr>; Jules Sanchez <jules.n.sanchez@gmail.com>
Subject: Re: EXPLANet: new results
 
Hi everyone,

I also agree with Giannini's argument. In addition, mAP evaluate only
one part of the model and not the whole model. Therefore, it makes more
sense to correlate SHAP-GED with the accuracy of the overall
classification model.


However, if we compare the old results of RetinaNet with the new ones,
it seems that when the accuracy of the overall model increases the SHAP
GED decreases.  Although, I would like to dig more into this interesting
point, I think that to be practical, we should work on finishing and
submitting the manuscript first.


Thank you all for the nice work
Best regards,
Siham


El 2021-01-20 00:13, Diaz Rodriguez Natalia escribió:
> hi Siham and Alberto,
>  here last experiments of Gianni, in the most fair way he could (same
> aggregating function, he could not have time to learn using a new
> cluster and so runned it with batch size 1), see email below.
>  Do you agree with this explanation?
>  [7]
>
> -------------------------
>
> From: Franchi Gianni <gianni.franchi@ensta-paris.fr>
> Sent: Tuesday, January 19, 2021 9:39 AM
> To: Diaz Rodriguez Natalia <natalia.diaz@ensta-paris.fr>; Jules
> Sanchez <jules.n.sanchez@gmail.com>
> Subject: new results
>
>  hello Natalia,
>
> Here is the results I get:
> Results on MONU AI
>
> ~ & mAP & Accuracy &SHAP GED
>  Faster R-CNN & $42.5$ & $86.8$ & $0.93$\\
>     \hline
>  RetinaNet (OLD results) &  $43.6$ & $87.3$ & $0.59$\\
>  RetinaNet (NEW results) &  $49.5$ & $90.4$ & $0.86$\\
>
> Result on Pascal part
> ~ & mAP & Accuracy &SHAP GED
>  Faster R-CNN &  $36.5$ & $82.4$ & $0.45$\\
>     \hline
>  RetinaNet (OLD results) &  $26.5$ & $79.7$ & $0.32$\\  RetinaNet (NEW
> results) &  $39.3$ & $80.3$ & $0.59$\\
>
>  I think now the results are better. since the accuracy is linked with
> the shap GED, but not the mAP.
>  This is in coherence with the fact that I dont think the more
> accurate the detector is (better mAP) => better GED,
>  because the mAP evaluates the spatial location AND the presence or
> not of a descriptor, while the GED evelautes just the presence.
>
>  best,
>
>  Gianni FRANCHI






El lun, 25 ene 2021 a las 17:51, Alberto Castillo Lamas (<alcasla90@gmail.com>) escribió:
Buenas Natalia.
Modificamos la formalización para que quedara más clara, pero ambas serían equivalentes, te puedo comentar el significado.
V contiene un v_i que sería la agregación de probabilidad para cada objeto i, como ves de 1 a 14 objetos/elementos arquitectónicos. Entonces v_1 si el 1 por ejemplo es el arco de medio punto, entonces sería la agregación de probabilidades de todas las detecciones cuya clase sea la 1. Realmente no podemos definir una matriz porque una dimensión (detecciones por clase) es variable debido a la salida del detector. Pueden salir 0 detecciones de una clase, o X, por eso en su momento preferimos formalizarlo de esa forma.

Me parece bien lo que habéis escrito. En vuestros términos: Si, N es un vector de 1 a n elementos. No se eliminan regiones, se tienen en cuenta todas las regiones del detector ya sean muy próximas a 0 o mayores (la agregación de las probabilidades era teniendo en cuenta todas las detecciones). Le sobre la frase de calcular p' (p prima). Resumiendo lo que ponéis esta bien excepto lo que te he comentado, N es un vector de n elementos, m son el número de regiones que salen del detector, p_m es un vector de escalares (probabilidad de cada región), y en N se hacen el acumulado como se dice.

Y como te comento, para la obtención del vector de probabilidades (N como lo llamas) no hay threshold. 

También algunos números que creo que están erróneos o no los he entendido mal (standard procedure table 6).


If I understood well your former version your notation where:

m is the number of object detected
n is the number of meta classes
i is a sub index over the meta classes
j is also a sub index over the meta classes (I am not sure about that one)


My notations:
M is the number of object detected
N is the number of meta classes
m is a sub index over the object detected
p_m and p'm are probality vector of size N that provides for every object detected the probability to belonging to one of the classes.


I corrected the document. 
What we agreed with Jules was done:



Let us consider one image with two objects O1 and O2, and let us consider that we have just three classes C1, C2 and C3. 



Faster RCNN and RetinaNet will both have the same output two vectors P1 and P2 of size three, where P1(1) is the proba of the class C1 for the first object, P1(2) is the proba of the class C2 for the first object , P1(3) is the proba of the class C3 for the first object. We can do the same for the second object and P2.

Alberto: Exactly.


Yet the Faster RCNN of torchvisio will transform P1 and P2 to P1' and P2', and we do not have access to P1 and P2.

What are these new vectors?

The transformation from P1 to P1, keeps the maximum probabilities of P1 and put the other to zero, let us say P1=[0.9,0.05,0.05]. Hence the function will transform P1 to P1'=[0.9,0,0]. 

Alb: I suppose you can specify the threshold to transforme lower values to 0, so using threshold=0 you will have all probabilities. If you cannot it doesn´t matter. As you said there is small difference.


Then, the Faster RCNN' code will aggregate the descriptor of the image D= P1' + P2'.

I did not manage to make such a function on RetinaNet. 

Hence the descriptor is D = P1+ P2. 

The difference is not that big since DNN are often overconfident. 




%future work: how important are spatial relations, asimetrias y otras caracteristicas geometricas.
%how to handle multiple style prediction instead of just predicting the predominant style?
% how many images for pix2pix orientation alignment?


If I understood well your former version your notation where:

m is the number of object detected
n is the number of meta classes
i is a sub index over the meta classes
j is also a sub index over the meta classes (I am not sure about that one)


My notations:
M is the number of object detected
N is the number of meta classes
m is a sub index over the object detected
p_m and p'm are probality vector of size N that provides for every object detected the probability to belonging to one of the classes.



[19:52, 1/29/2021] Gianni Franchi: On utilise overall accuracy comme tout le monde et dans le monde du deep Learning cela s’appelle accuracy. L’autre accuracy c’est l’average accuracy et on ne fait pas ça
[19:53, 1/29/2021] Gianni Franchi: On fait comme tout le monde en deep learning avec les bonnes appellations du deep learning
[20:04, 1/29/2021] Natalia: Dont know why we have the othet one lol
[20:06, 1/29/2021] Gianni Franchi: It is OOD machine learning people that use both. It is useful if the dataset is imbalanced, but more and more no one evaluate the average accuracy....
[20:08, 1/29/2021] Natalia: to be clear we use 11 or 12?
[20:09, 1/29/2021] Gianni Franchi: What is 11 and what is 12?
[20:09, 1/29/2021] Gianni Franchi: I got it.
I told you we use 11 like everyone in deep learning
% \begin{align}
%     \label{ec:precrecf1}
%     \begin{split}
%         accuracy &= \frac{\#correct\ predictions}{\#total\ predictions} \\
%     \end{split}
% \end{align}


%Multi-class classification accuracy
% \begin{align}
%     \label{ec:precrecf1}
%     \begin{split}
%         accuracy &= \frac{TP+TN}{\#total\  predictions} \\
%     \end{split}
% \end{align}

[08:44, 2/1/2021] Natalia: we cannot  say we do a process or methodology that is end-to-end, am I right? due to the training of one model, shap computation, training again, etc...coul dit be automated for an end to end methodology?
[11:39, 2/1/2021] Natalia: we say right now:


EXPLANet, a new  end-to-end deep learning (DL) architecture for compositional part-based detection and classification. The design of this network was guided to align with expert knowledge.
[16:19, 2/1/2021] Jules Sanchez: Hum end to end is ambiguous.
Gianni can confirm, but usually end to end means that everything can be traines with one "generalized" backward pass.
Here due to some non derivable computation (shap), or disjoint model (detection and classification are trained seperately), it is hardly end to end.
But it could be fully automated nonetheless.



Figure:
[11:47, 2/2/2021] Jules Sanchez: XAI loss as output of neural processing is weire because it needs the symbolic processing to do it.
L_SHAP comes from neural processing + symbolic processing
[11:48, 2/2/2021] Natalia: you are totally right
[11:48, 2/2/2021] Natalia: i ll add two clouds of 2 different losses
[11:48, 2/2/2021] Natalia: that are merged and processed in the purple box
[11:48, 2/2/2021] Jules Sanchez: Yes it is merged in the xai procedure !
[11:49, 2/2/2021] Jules Sanchez: You could have first cloud "neural loss" and a cloud behind symbolic processing with "miscontribution" or something like that
[12:00, 2/2/2021] Natalia: i like term Neural loss!! merci!
[12:01, 2/2/2021] Natalia: behind you mean inside? or to the right?
[12:02, 2/2/2021] Jules Sanchez: I'm not sure how you want to represent it. But it is basically the output of the sumbolic processing for us
[12:10, 2/2/2021] Natalia: smth like this no?
[12:11, 2/2/2021] Jules Sanchez: Yes it is better 
[12:13, 2/2/2021] Natalia: maybe i mention an example of neural loss
[12:14, 2/2/2021] Jules Sanchez: Hum. Yes, we use cross entropy loss for classification fir instance (I think)







RELATED WORK REMOVED: too verbose:


	\textit{LIME} \cite{ribeiro2016should} is a technique that explains the prediction by learning a local interpretable model around the prediction. The proposed approach limits itself to linear models as local interpretable models. This method can be seen as an attribution method, as it tries to gauge the importance of the input feature with the final prediction. %We could think of expanding this class of models for the optimization step. #futureWork	
When applied to images, LIME divides the input image into superpixels (such as SLIC \cite{achanta2012slic}) as they tend to have more meaningful information than singular pixels for a human audience. The output consists of the superpixels that contribute the most to a specific class (a \textit{factual} explanation). This idea can be expanded to superpixels that contribute negatively to the output.

